Towards Information-Seeking Agents

We develop a general problem setting for training and testing the ability of agents to gather information efficiently. Specifically, we present a collection of tasks in which success requires searching through a partially-observed environment, for fragments of information which can be pieced together to accomplish various goals. We combine deep architectures with techniques from reinforcement learning to develop agents that solve our tasks. We shape the behavior of these agents by combining extrinsic and intrinsic rewards. We empirically demonstrate that these agents learn to search actively and intelligently for new information to reduce their uncertainty, and to exploit information they have already acquired.

==> UCI.tex <==
Moving away from images and convolutional architectures, we next present several results for the problem of \emph{cost sensitive classification}. Performance in this task is measured in terms of how well a model can trade off between feature evaluation costs and making correct decisions. 

==> lightintro.tex <==
% What's information seeking
% 

Humans possess an innate desire to know and to understand.
To do so, we seek information actively through behaviors both simple (glancing at a billboard) and elaborate (conducting scientific experiments)~\citep{gottlieb2013}.
Abstractly, information seeking is based around querying an \emph{information source} -- which may be a human,  machine, or other part of the environment -- in order to satisfy an information need, to perform a specific task, or perhaps simply out of \emph{curiosity} (which can be considered as an unconscious precursor to the need [REF]).
It is an high-level cognitive process that is peculiar to humans (and to some particularly clever animals) and it allows us to better deal with a complex, ever-changing environment.
Artificial agents could benefit greatly from similar capacities.

%
In this paper, we aim to seed the development of artificial agents that learn how to ask for the information they need in order to solve a task.
Therefore, we posit that there is an environment, i.e. an information source detaining the knowledge, which is hidden from the agent.
The task of the agent is to iteratively interact with the information source in order to obtain salient bits of information (clues).
We assume that the form of this interaction is usually regulated by an interface, e.g. a language, exposed by the information source: the agent needs to formulate questions interpretable and answerable by the source.
A desiderata of the agent is to perform this interaction efficiently.
We are particularly interested in information efficiency, as measured by the amount of bits transferred from the source.

Humans focus attention selectively to acquire information when and where it is needed~\citep{rensink2000}. The setting in which an agent progressively acquires pieces of information is similar in spirit to previous \emph{attention} models applied to vision tasks~\cite{ram, draw, ranzato2014}.
Here, we want to encourage a shift in perspective and interpret attention as a special case of question asking.


We build several tasks around existing datasets, including cluttered MNIST~\citep{ram} and the annotated face corpus CelebA~\citep{celeba}.
On MNIST, our model learns to classify the digit only by asking for a small portion of the overall image. On CelebA, we tackle a conditional classification problem, in which the model learns to assess if the input image has a given annotation under a similar budgeted regime. 
%In these tasks, each question consists of asking for the value of a particular set of pixels.
We also develop tasks based on datasets of our own design, including a visual BlockWorld and a character-level text-based game. Using techniques from deep learning and reinforcement learning, we show how agents can be trained end-to-end to complete our tasks. Overall, we adopt a reinforcement learning perspective, characterizing the environment as an information source and an agent's actions as questions that selectively extract information from the environment.

\begin{figure}[tbp]
\centering
\includegraphics[scale=0.53]{imgs/celebacondclass.png}
\caption{Example behavior of an information-seeking agent for a conditional question answering task on CelebA, while trying to assess the truth value of the attribute ``male'' in the input image (top row). The second row shows the distribution over which pixels the model will ask about next. The third row contains what the model already saw. The fourth row is the confidence of the model in the answer (darker color corresponds to a negative answer). The model initially forms an incorrect belief, but quickly corrects that belief after obtaining further information.}
\end{figure}


\subsection{The importance of attention}

%%%%% NEW-PARAGRAPH
Information seeking is closely related to the concept of \emph{attention}.
~\citet{rensink2000} points out that humans focus attention selectively to acquire information when and where it is needed, and combine attentive fixations to build an internal representation of the environment.
Figure 1 shows the behavior of our model on CelebA, trying to infer whether or not the subject in the picture is a man or a woman.
Iteratively, the model asks the environment to uncover small image patches following its learnt belief on how important will be the received information.

The subject of attention in neural models has become prominent in recent years~\citep{bahdanau2014,iaa}, and is preceded by earlier work~\citep{larochelle2010}. Learning where to look was also investigated in~\citet{ranzato2014},~\citet{ram} and~\citet{draw}.~\citet{draw} use attention to improve the generation of visual data, while~\citet{ram} seek to mitigate the computational cost of visual classification by ignoring parts of the input image.

In our case, attentive behavior arises from the constraints one put on the maximum amount of information that can be transferred at each step, from the type of questions that can be asked, and from the demand that the agent minimize the number of question asked prior to task solution.
In the aforementioned example, this information efficiency requirement may be quantified with the number of pixels that the model peeks at.


Conceptually, we extend the concept of attention to the more general concept of question-asking, which is applicable in a broader setting (consider for example the case in which the information source is adversarial, i.e. when the result of the attention step is a distorted or noisy version of the world).



==> misc_background.tex <==
%%%%% NEW-PARAGRAPH


Closely related is the concept of \emph{attention}.

~\citet{rensink2000} points out that humans focus attention selectively to acquire information when and where it is needed, and combine attentive fixations to build an internal representation of the environment.
This is the standpoint of the well-known works of~\citet{ranzato2014},~\citet{ram} and~\citet{draw}, that develop neural models to ``learn where to look'' in the context of visual scenes.~\citet{draw} seek to improve the generation of visual data. ~\citet{ram} is closer to our work and learn how to take ``glimpses'' of an image in order to mitigate the computational cost for image classification.
In this paper, our focus is to use attention as a strategy to minimize the amount of information transmitted between the source and the agent. Conceptually, we extend the concept of attention to question-asking, which may be more suitable in the case of adversarial environments (i.e. when the result of the attention step is a distorted, or noisy version of the world) or human exchanges.




%Endowing artificial agents with such capacities is a suitable achievement. Such agents may be used in natural language dialog settings, in which the agent need to infer the state of the user for slot-filling tasks [REF] or for recommendation [REF]. Used in one-shot learning to get which question remains to ask ? which element to show next ? some ideas here ?

%In this work, we abstract the notion of a question by means of some toy task where we interpret a question as a means to access the hidden environment. (say here that attention is a particular type of question that always show what's underneath the environment ?). (add references to RAM and distantiate our model from that).

%A crucial requirement for effective information-seeking is efficiency.
%We assume that the communication channel between the agent and the information source is (a) restricted in capacity, in the sense that all the information cannot be transmitted at once, and (b) costly, which motivates the agent to gather the information as quickly as possible.

% Information seeking is closely related to the concept of \emph{attention}. \citet{rensink2000} points out that humans focus attention selectively to acquire information when and where it is needed, and combine attentive fixations to build an internal representation of the environment. Similarly, attention can improve efficiency because irrelevant features outside of attended regions are naturally ignored~\citep{ram}. Attention and information seeking are distinct from other acts carried out by agents in that they do not affect the external world {\it per se}, but rather alter an agent's epistemic state~\citep{gottlieb2013}.

% The subject of attention in neural models has become prominent in recent years \citep{bahdanau2014,ranzato2014,draw,ram,iaa}, and is preceded by earlier work~\citep{larochelle2010}. In particular,~\citet{draw} and~\citet{ram} develop neural models that ``learn where to look'' to improve their understanding of visual scenes. This is closely related to our problem setting, but differs in details and motivation.~\citet{draw} seek to improve the generation of visual data, while~\citet{ram} seek to mitigate the computational cost of visual classification.

% Beyond autoregressive behavior, \emph{20 Questions} highlights (and exaggerates) the limited-capacity communication channel that restricts real-world information seeking.  This is partly why humans must be efficient in their search for information and why we impose similar restrictions in <NAME>.
% Almost all ``guessing games'', from \emph{20 Questions} to \emph{Battleship} to \emph{Hangman}, seem expressly designed to train efficient information seeking, or at least to exploit humans' intrinsic joy in exercising it.
% It was the consideration of guessing games that originally motivated our research. There exists an inherent link between experimentation and the questioning involved in such games, since an experiment can be viewed as a question that is asked of the environment.



==> oldintro.tex <==
% What's information seeking
% 

Humans possess an innate desire to know and to understand.
To do so, we seek information actively through behaviors both simple (glancing at a billboard) and elaborate (conducting scientific experiments)~\citep{gottlieb2013}.
\emph{Information-seeking} behaviors can be defined as those in which humans purposefully engage in order to change their state of knowledge [REF].
Abstractly, information seeking is based around querying an \emph{information source} -- which may be a human,  machine, or other part of the environment -- in order to satisfy an information need, to perform a specific task, or perhaps simply out of \emph{curiosity} (which can be considered as an unconscious precursor to the need [REF]).
Information seeking is a general, exploratory, and iterative process that comprises formulating hypotheses, retrieving information, and refining hypotheses based on the acquired information.
This high-level cognitive process is peculiar to humans (and some particularly clever animals) and it allows us to better deal with a complex, ever-changing environment. Artificial agents could benefit greatly from similar capacities.

%
One fundamental aspect of successful information-seeking is \emph{efficiency}.
Usually, the communication channel between the agent and the information source is costly and a desirable behaviour is to minimize the number of exchanges or the number of bits of information that have been transmitted. Moreover, a typical information-seeking scenario is characterized by various restrictions such as the limited perceptive capabilities of the agent, the transport capacity of the communication channel, or the fixed interface through which information may be obtained from the source. In this setting, it is important for the agent to find an efficient strategy for acquiring relevant information.

%
In this paper, we aim to further the development of information-seeking agents by formulating a collection of tasks whose solution requires efficient acquisition and integration of information.
The tasks vary in difficulty, but all involve questioning an information source iteratively in order to obtain salient bits of information (clues). Crucially, we strongly restrict the interaction between the agent and the information source by limiting both the number of questions that can be asked and the amount of information that can be extracted from the source at each turn. Moreover, we consider the source as a black-box endowed with a fixed interface (e.g. a set of possible questions) through which information may be obtained. These choices are intended to make our tasks more similar to real-world scenarios, for example dialog, in which humans seek for information by formulating questions in a specific language. Overall, we frame the goal of the agent as learning a policy for asking questions that efficiently gather sufficient information to solve a task.

We build several tasks around existing datasets, including cluttered MNIST~\citep{ram} and the annotated face corpus CelebA~\citep{celeba}.
On MNIST, our model learns to classify the digit only by asking for a small portion of the overall image. On CelebA, we tackle a conditional classification problem, in which the model learns to assess if the input image has a given annotation under a similar budgeted regime. 
%In these tasks, each question consists of asking for the value of a particular set of pixels.
We also develop tasks based on datasets of our own design, including a visual BlockWorld and a character-level text-based game. Using techniques from deep learning and reinforcement learning, we show how agents can be trained end-to-end to complete our tasks. Overall, we adopt a reinforcement learning perspective, characterizing the environment as an information source and an agent's actions as questions that selectively extract information from the environment.

\begin{figure}[tbp]
\centering
\includegraphics[scale=0.53]{imgs/celebacondclass.png}
\caption{Example behavior of an information-seeking agent for a conditional question answering task on CelebA, while trying to assess the truth value of the attribute ``male'' in the input image (top row). The second row shows the distribution over which pixels the model will ask about next. The third row contains what the model already saw. The fourth row is the confidence of the model in the answer (darker color corresponds to a negative answer). The model initially forms an incorrect belief, but quickly corrects that belief after obtaining further information.}
\end{figure}

%This paper is organized as follows. In Section~\ref{sec:prob} we formally define the general information-seeking problem setting and the particular tasks to be solved. In Section~\ref{sec:model} we describe the models we have devised to realize information-seeking behavior. Section~\ref{sec:exp} details our experimental results (with analysis). We conclude in Section~\ref{sec:conc}.

\subsection{The importance of attention}

%%%%% NEW-PARAGRAPH
Information seeking is closely related to the concept of \emph{attention}.
~\citet{rensink2000} points out that humans focus attention selectively to acquire information when and where it is needed, and combine attentive fixations to build an internal representation of the environment.
Figure 1 shows the behavior of our model on CelebA, trying to infer whether or not the subject in the picture is a man or a woman.
Iteratively, the model asks the environment to uncover small image patches following its learnt belief on how important will be the received information.

The subject of attention in neural models has become prominent in recent years~\citep{bahdanau2014,iaa}, and is preceded by earlier work~\citep{larochelle2010}. Learning where to look was also investigated in~\citet{ranzato2014},~\citet{ram} and~\citet{draw}.~\citet{draw} use attention to improve the generation of visual data, while~\citet{ram} seek to mitigate the computational cost of visual classification by ignoring parts of the input image.

In our case, attentive behavior arises from the constraints one put on the maximum amount of information that can be transferred at each step, from the type of questions that can be asked, and from the demand that the agent minimize the number of question asked prior to task solution.
In the aforementioned example, this information efficiency requirement may be quantified with the number of pixels that the model peeks at.


Conceptually, we extend the concept of attention to the more general concept of question-asking, which is applicable in a broader setting (consider for example the case in which the information source is adversarial, i.e. when the result of the attention step is a distorted or noisy version of the world).


% Conceptually, instead of ignoring information in an environment that is fully observable (if that was indeed the best approach), information seeking needs to gather useful information from a system that is observable only by means of a restricted set of questions. We explicitly treat the information source as a black-box, in which the mechanism underlying the answer generation is non-observable.
% We extend the concept of attention to the more general concept of question-asking, which is applicable in a broader setting (consider for example the case in which the information source is adversarial, i.e. when the result of the attention step is a distorted or noisy version of the world).


% \subsection{The information-seeking agent}
% We consider that information-seeking agents are composed of two main interacting components: a question generation component and a memory component.
% The question generation component is responsible for synthesising a request and interacting with the information source;
% The memory component is responsible for organizing the results retrieved from the information source.



% Usually, memorization and communication is costly. In order to minimize memory/information-stocking and communication costs intelligent policy/inference is needed. Efficiency is a keyword here. Humans try to do things / structure communication efficiently (is that true ? :-D) (edited)
%The signal that drives the learning process can either come from:
%a)  a specific task / satisfy a specific information need (IR related concept)
%b)  a curiosity-based "reward", in which the agent tries to _efficiently_ gather a representation of the environment (edited)
%The communication channel between the agent and the information source is usually constrained and it's structured as a language L (difference with set of actions ?). (edited)
%Usually, the language is specified by the information source, akin to the possible actions that one can perform in an environment from a RL perspective.



==> oldmodel.tex <==
We address the information seeking problem by developing a family of models which ask sequences of simple questions and combine the resulting answers in order to minimize the amount of information consumed while solving various tasks. The ability to actively integrate received knowledge into some sort of memory is potentially extremely useful, but we do not focus on that ability in this paper. For the present work, we focus strictly on whether a model can effectively reason about observed information in a way that reduces the number of questions asked while solving a task. We assume that a model records all previously asked questions and their corresponding answers, perhaps in a memory whose structure is well-suited to the task-at-hand.
%We now provide a more formal description of our general task objective, the techniques we use to train our models, and some model architectures designed for particular tasks.

\subsection{An Objective for Information-Seeking Agents}
\label{sec:model_objective}
We formulate our objective as a sequential decision making problem. At each decision step, the model considers the information it has received up until the current step, and then selects a particular question from among a set of questions which it can ask of the environment. Concurrently, the model formulates and refines a prediction about some unknown aspect(s) of the environment. E.g., while sequentially selecting pixels to observe in an image, the model attempts to predict whether or not the person in that image is wearing a hat.

For the current paper, we make two main simplifying assumptions: (1) the answer to a given question will not change over time and (2) we can precisely remember previous questions and answers. Assumption (1) holds (at least approximately) in many useful settings and (2) is easily achieved with modern computers. Together, these assumptions allow us to further simplify the problem by eliminating previously-asked questions from consideration at subsequent time steps.

While the precise objectives we consider vary from task-to-task, they all follow the same pattern:
\begin{equation}
\maximize_{\theta} \expect_{(x, y) \sim \DD} \left[ \expect_{\{(q_1, a_1),...,(q_T, a_T)\} \sim (\pi_{\theta}, O, x)} \left[ \sum_{t=1}^{T} R_t(f_{\theta}(q_1, a_1, ..., q_t, a_t), x, y) \right] \right].
\label{eq:task_obj_general}
\end{equation}
In Eqn.~\ref{eq:task_obj_general}, $\theta$ indicates the model parameters and $(x, y)$ denotes an \emph{observable}/\emph{unobservable} data pair sampled from some distribution $\DD$.
We assume questions \emph{can} be asked about $x$ and can \emph{not} be asked about $y$. $\{(q_1, a_1),...,(q_T, a_T)\}$ indicates a sequence of question/answer pairs generated by allowing the policy $\pi_{\theta}$ to ask $T$ questions $q_t$ about $x$, with the answers $a_t$ provided by an observation function $O(x, a_t)$\footnote{I.e., we may be unable to backprop through $O(x, a)$, though its derivatives could be useful when available.}. 
$R_t(f_{\theta}(\cdot), x, y)$ indicates a (possibly) non-stationary task-specific reward function which we assume to be a deterministic function of the model's \emph{belief state} $f_{\theta}(\cdot)$ at time $t$, and the observable/unobservable data $x$/$y$. For our tasks, $R_t$ is differentiable with respect to $f_{\theta}$, but this is not required in general.
Intuitively, Eqn.~\ref{eq:task_obj_general} says the agent should ask questions about $x$ which most quickly allow it to make good predictions about $x$ and/or $y$, as measured by $R_t$.

As a concrete example, $(x, y)$ could be an image/annotation pair sampled from $\DD \equiv \mbox{CelebA}$, each question $q_t$ could indicate a 4x4 block of pixels in $x$, $O(x, q_t)$ could provide the value of those pixels, and $R_{t}$ could be the log-likelihood which the model's belief state $f_{\theta}$ assigns to the true value of $y$ after observing the pixels requested by questions $\{q_1, ..., q_t\}$ (i.e.~$\{a_1,...,a_t\}$).

\subsection{Training}
\label{sec:model_training}

We train our models using Generalized Advantage Estimation (\cite{schulman2016}, abbr.~GAE), TD($\lambda$) (\cite{sutton1998}), and standard backpropagation.
We use GAE to train our models how to \emph{make better decisions}, TD($\lambda$) to train the value function approximators required by GAE, and backpropagation to train our models how to \emph{cope with their decisions}. When the observation function $O(x, q_t)$ is differentiable w.r.t.~$q_t$ and the policy $\pi_{\theta}(q_t | h_{:t})$ has a suitable form, GAE and TD($\lambda$) can be replaced with a significantly lower variance estimator based on the ``reparametrization trick'' \citep{kingma2014, rezende2014, silver2014}.

We train our models by stochastically ascending an approximation of the gradient of Eqn.~\ref{eq:task_obj_general}.
Considering a fixed $(x, y)$ pair -- incorporating the expectation over $(x, y) \sim \DD$ is simple --
the gradient of Eqn.~\ref{eq:task_obj_general} w.r.t.~$\theta$ can be written:
\begin{align}
\nabla_{\theta} \expect_{\{(q_t, a_t)\} \sim (\pi_{\theta}, O, x)}& \left[ \sum_{t=1}^{T} R_t(f_{\theta}(q_1, a_1, ..., q_t, a_t), x, y) \right] = \nonumber \\
\expect_{\{(q_t, a_t)\} \sim (\pi_{\theta}, O, x)}& \left[ \sum_{t=1}^{T} \left( \nabla_{\theta} \log \pi_{\theta}(q_t | h_{:t}) R_{t:} + \nabla_{\theta} R_t(f_{\theta}(h_{:t+1}), x, y) \right) \right], \label{eq:obj_grad_full}
\end{align}
in which $R_{t:}$ refers to the total reward received after asking question $q_t$, and $h_{:t}$ indicates the history of question/answer pairs $\{(q_1,a_1),...,(q_{t-1},a_{t-1})\}$ observed prior to asking question $q_t$.

The gradient in Eqn.~\ref{eq:obj_grad_full} can be interpreted as comprising two parts:
\begin{align}
\nabla_{\theta}^{\pi} \equiv& \expect_{\{(q_t, a_t)\} \sim (\pi_{\theta}, O, x)} \left[ \sum_{t=1}^{T} \nabla_{\theta} \log \pi_{\theta}(q_t | h_{:t}) (R_{t:} - V_{\theta}(h_{:t})) \right] \;\;\;\; \mbox{and} \label{eq:obj_grad_decide} \\
\nabla_{\theta}^{f} \equiv& \expect_{\{(q_t, a_t)\} \sim (\pi_{\theta}, O, x)} \left[ \sum_{t=1}^{T}  \nabla_{\theta} R_t(f_{\theta}(h_{:t+1}), x, y) \right], \label{eq:obj_grad_cope}
\end{align}
where we have introduced the approximate value function (i.e.~baseline) $V_{\theta}(h_{:t})$.
Roughly speaking, $V_{\theta}(h_{:t})$ provides an estimate of the expectation of $R_{t:}$ and is helpful in reducing variance of the gradient estimator in Eqn.~\ref{eq:obj_grad_decide} \citep{sutton1998}.
Intuitively, $\nabla_{\theta}^{\pi}$ modifies the distribution of question/answer sequences $\{(q_1, a_1),...,(q_T, a_T)\}$ experienced by the model, and $\nabla_{\theta}^{f}$ makes the model better at predicting given the current distribution of experience.
Respectively, $\nabla_{\theta}^{\pi}$ and $\nabla_{\theta}^{f}$ train the model to make better decisions and to cope with the decisions it makes.

%%%%%
We estimate $\nabla_{\theta}^{f}$ directly using standard backpropagation and Monte Carlo integration of the required expectation.
In contrast, obtaining useful estimates of $\nabla_{\theta}^{\pi}$ is quite challenging and a subject of ongoing research.
%The direct Monte Carlo estimate of this gradient is prone to high variance due to the sum over many random variables which produces $R_{t:}$.
We use the GAE estimator presented by \cite{schulman2016}, which takes a weighted average of all possible $k$-step actor-critic estimates of $R_{t:}$.
Each of the $k$-step actor-critic estimates of $R_{t:}$, which we denote $\hat{R}_{t:}^{k}$, is computed as follows:
\begin{equation}
\hat{R}_{t:}^{k} \equiv \gamma^{k} V_{\theta}(h_{:t+k}) + \sum_{t^{\prime} = t}^{t + k - 1} \gamma^{t^{\prime} - t} R_{t^{\prime}}(f_{\theta}(h_{:t^{\prime}+1}), x, y), \label{eq:k_step_ac}
\end{equation}
in which $\gamma$ is a reward discounting factor and $k > 0$ gives the number of Monte Carlo roll-out steps.
The estimator in Eqn.~\ref{eq:k_step_ac} allows the policy $\pi_{\theta}$ to act and collect rewards from the environment for $k$ steps, after which the roll-out is truncated and subsequent rewards are estimated using the approximate value function $V_{\theta}(h_{:t+k})$.
Given the $k$-step actor-critic estimates of $R_{t:}$ in Eqn.~\ref{eq:k_step_ac}, the GAE estimator for $\nabla_{\theta}^{\pi}$ is given by:
\begin{equation}
\hat{\nabla}_{\theta}^{\pi} \equiv \expect_{\{(q_t, a_t)\} \sim (\pi_{\theta}, O, x)} \left[ \sum_{t=1}^{T} \nabla_{\theta} \log \pi_{\theta}(q_t | h_{:t}) \left(-V_{\theta}(h_{:t}) + (1 - \lambda) \sum_{k=1}^{T-t} \lambda^{k-1} \hat{R}_{t:}^{k} \right) \right], \label{eq:gae_estimator}
\end{equation}
in which $0 < \lambda < 1$ is an additional hyperparameter. Note that the estimator in Eqn.~\ref{eq:gae_estimator} assumes a long horizon $T$ for which $(1 - \lambda) \sum_{k=1}^{T-t} \lambda^{k-1} \approx 1$. The horizon in our tasks is relatively short (between 10 and 100), and some adjustment is required to maintain the property of taking a weighted average of truncated actor-critic estimates of $R_{t:}$. Details are available in the supplementary material.

The GAE estimator in Eqn.~\ref{eq:gae_estimator} requires an approximate value function $V_{\theta}(h_{t:})$. We train $V_{\theta}(h_{:t})$ by minimizing the expected squared TD($\lambda$) error given by:
\begin{equation}
\mbox{ERR}_{\mbox{TD}(\lambda)} \equiv \expect_{\{(q_t, a_t)\} \sim (\pi_{\theta}, O, x)} \left[ \sum_{t=1}^{T} \left( V_{\theta}(h_{:t}) - (1 - \lambda) \sum_{k=1}^{T-t} \lambda^{k-1} \hat{R}_{t:}^{k} \right)^2 \right]. \label{eq:tdl_error}
\end{equation}
As is typical for TD($\lambda$), we backpropagate through $V_{\theta}(h_{:t})$ in Eqn.~\ref{eq:tdl_error}, but not through $\hat{R}_{t:}^{k}$.

\subsection{Model Architectures for Information Seeking}
\label{sec:model_architecture}

\begin{figure}
\vspace{-0.1cm}
\begin{center}
  \subfigure[]{\includegraphics[scale=0.42]{./imgs/agent_net_conv.pdf} \vspace{-0.2cm}}
  \subfigure[]{\includegraphics[scale=0.42]{./imgs/agent_net_fc_vert_pad.pdf} \vspace{-0.2cm}}
\caption{The network architectures developed for (a) our experiments with images and (b) our experiments with permutation-invariant data. We describe how computation proceeds through these architectures at each step of a trial in Section~\ref{sec:model_architecture}. The current trial history $h_{:t}$ is input to (a) through the bottom-up network. The values $f_{\theta}^{x}(h_{:t})$, $f_{\theta}^{y}(h_{:t})$, $V_{\theta}(h_{:t})$, and $\pi_{\theta}(q_t | h_{:t})$ are collected from the indicated locations. We use $f_{\theta}^{x,y}$ to denote a model's predictions about the complete observable data $x$ and the unobservable data $y$. Computation in architecture (b) proceeds from bottom to top, starting with the history input $h_{:t}$ and then passing through several fully-connected layers linked by shortcut connections. The values $f_{\theta}^{x}(h_{:t})$, $f_{\theta}^{y}(h_{:t})$, $V_{\theta}(h_{:t})$, and $\pi_{\theta}(q_t | h_{:t})$ are computed as linear functions of the output of the shared network.}
\label{fig:model_figs}
\end{center}
\vspace{-0.1cm}
\end{figure}

We use deep neural networks to represent the functions $\pi_{\theta}$, $f_{\theta}$, and $V_{\theta}$ described in the preceding sections. Our networks share parameters extensively. Figure~\ref{fig:model_figs} illustrates the specific architectures we developed for tasks involving images and generic data.
For the tasks we examine, the number of possible questions is moderately sized, i.e.~$< 1000$, and the possible answers to each question can be represented by small vectors, or perhaps even single scalars. Additionally, the response to a particular question will always have the same type, i.e.~if question $q_t$ produces a 4d answer vector $a_t \equiv O(x, q_t)$ for some $x$, then it produces a 4d answer vector for all $x$.

Given these assumptions, we can train neural networks whose inputs are tables of (qrepr, answer) tuples, where each tuple provides the answer to a question (if it has been asked), and a \emph{question representation}, which provides information about the question which was asked.
E.g., a simple question representation might be a one-hot vector indicating which question, among a fixed set of questions, was asked.
Our networks process the tables summarizing questions and answers which they have observed so far (i.e.~a trial history $h_{:t}$) by vectorizing them and feeding them through one or more hidden layers.
We compute quantities used in training from one or more of these hidden layers -- i.e.~the value function estimate $V_{\theta}(h_{:t})$, the policy $\pi_{\theta}(q_t | h_{:t})$, and the belief state $f_{\theta}(h_{:t})$.

%More precisely, at each time step $t$ in a given trial, the model must compute: (1) $\pi_{\theta}(q_t | h_{:t})$ -- a distribution over which question to ask next, (2) $f_{\theta}(h_{:t})$ -- a prediction about some aspect(s) of the environment conditioned on the questions/answers observed at times $1...t-1$, and (3) $V_{\theta}(h_{:t})$ -- an estimate of future rewards for use during training.
%Note that, during training, the values of $f_{\theta}(h_{:t})$ and $V_{\theta}(h_{:t})$ which respond to the question $q_t$ are offset from the selection of that question by $\pi_{\theta}(h_{:t})$ by one time step -- see subscripts.

The architecture in Fig.~\ref{fig:model_figs}a first evaluates a \emph{bottom-up} network comprising a sequence of convolutional layers topped by a fully-connected layer.
Each convolutional layer in this network performs 2x downsampling via strided convolution.
For the fully-connected layer we use an LSTM \citep{hochreiter1997}, which maintains internal state from step to step during a trial. 
After computing the output of each layer in the bottom-up network, we then evaluate a sequence of layers making up the \emph{top-down} network.
Each layer in the top-down network receives input both from the preceding layer in the top-down network and a partner layer in the bottom-up network (see arrows in (a)).
Each convolutional layer in the top-down network performs 2x upsampling via strided convolution.

The input to the bottom-up network is an image, masked to reveal only the pixels whose value the model has previously queried, and a bit mask indicating which pixels are visible. 
The output of the top-down network has the same spatial shape as the input image, and provides both a reconstruction of the \emph{complete} input image and the values used to compute $\pi_{\theta}(q_t | h_{:t})$.
The value function $V_{\theta}(h_{:t})$ at time $t$ is computed as a linear function of the bottom-up network's LSTM state.
For labelling tasks, the class prediction $f_{\theta}^{y}(h_{:t})$ is computed similarly.
The input reconstruction $f_{\theta}^{x}(h_{:t})$ is taken from the top-down network's output.
The policy $\pi_{\theta}(h_{:t})$ is computed by summing pixel-level values from a single channel in the top-down network's output over regions whose pixels the model has yet to ask about.
A softmax is applied to the summed pixel-level values to get the final probabilities for which pixels the model will ask about next.

The fully-connected architecture in Fig.~\ref{fig:model_figs}b performs similar computations to the convolutional architecture. The input to this model is an observation vector, masked to reveal only the features which have already been requested by the model, and a mask vector indicating which features have been requested. These vectors are concatenated and fed through a sequence of four shared hidden layers linked by shortcut connections. The values $f_{\theta}^{x}(h_{:t})$, $f_{\theta}^{y}(h_{:t})$, $V_{\theta}(h_{:t})$, and $\pi_{\theta}(q_t | h_{:t})$ are all computed as linear functions of the output of the final shared layer, with a softmax used to make $\pi_{\theta}(q_t | h_{:t})$ a distribution over which feature to request next.

We use Leaky ReLU activation functions throughout our networks, and apply layer normalization in all hidden layers to deal with the variable input magnitude caused by large variation in the number of visible pixels/features over the course of a trial. Layer weights are all initialized with a basic orthogonal init. We use the ADAM optimizer \citep{kingma2015} in all our tests, while working with minibatches of 100 examples each.
